Does Long-Term Series Forecasting Need Complex Attention and Extra Long Inputs?

As Transformer-based models have achieved impressive performance on various time series tasks, Long-Term Series Forecasting (LTSF) tasks have also received extensive attention in recent years. However, due to the inherent computational complexity and long sequences demanding of Transformer-based methods, its application on LTSF tasks still has two major issues that need to be further investigated: 1) Whether the sparse attention mechanism designed by these methods actually reduce the running time on real devices; 2) Whether these models need extra long input sequences to guarantee their performance? The answers given in this paper are negative. Therefore, to better copy with these two issues, we design a lightweight Period-Attention mechanism (Periodformer), which renovates the aggregation of long-term subseries via explicit periodicity and short-term subseries via built-in proximity. Meanwhile, a gating mechanism is embedded into Periodformer to regulate the influence of the attention module on the prediction results. Furthermore, to take full advantage of GPUs for fast hyperparameter optimization (e.g., finding the suitable input length), a Multi-GPU Asynchronous parallel algorithm based on Bayesian Optimization (MABO) is presented. MABO allocates a process to each GPU via a queue mechanism, and then creates multiple trials at a time for asynchronous parallel search, which greatly reduces the search time. Compared with the state-of-the-art methods, the prediction error of Periodformer reduced by 13% and 26% for multivariate and univariate forecasting, respectively. In addition, MABO reduces the average search time by 46% while finding better hyperparameters. As a conclusion, this paper indicates that LTSF may not need complex attention and extra long input sequences. The code has been open sourced on Github.

==> texes/bios.tex <==
% \appendices
% \section{Proof of the First Zonklar Equation}
% Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
% \section{}
% Appendix two text goes here.


% use section* for acknowledgment
% \ifCLASSOPTIONcompsoc
%   % The Computer Society usually uses the plural form
%   \section*{Acknowledgments}
% \else
%   % regular IEEE prefers the singular form
%   \section*{Acknowledgment}
% \fi


% The authors would like to thank...


% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
% \ifCLASSOPTIONcaptionsoff
%   \newpage
% \fi

\vfill
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/MyPhoto.jpg}}]{Daojun Liang}
  received the B.S. degree in computer science from Taishan University, China, in 2016, and the M.S. degree from the School of Information Science \& Engineering from the Shandong Normal University, Jinan, China, in 2019. He is currently pursuing the Ph.D. degree with the School of Information Science and Engineering, Shandong University, Jinan, China.
  His research interests include deep learning, machine learning, time series forecasting and federated learning.
\end{IEEEbiography}
\vfill

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/HaixiaZhang.jpg}}]{Haixia Zhang}(Senior Member, IEEE) received the B.E. degree from the Department of Communication and Information Engineering, Guilin University of Electronic Technology, China, in 2001, and the M.Eng. and Ph.D. degrees in communication and information systems from the School of Information Science and Engineering, Shandong University, China, in 2004 and 2008, respectively. From 2006 to 2008, she was an Academic Assistant at the Institute for Circuit and Signal Processing, Munich University of Technology. From 2016 to 2017, she was a Visiting Professor with the University of Florida, USA. She is currently a Distinguished Professor with Shandong University. Her current research interests include industrial Internet of Things (IIoT), resource management, mobile edge computing, and smart communication technologies. She serves as a TPC member, a session chair, an invited speaker and a keynote speaker for conferences. She is on the Editorial Boards of the \textit{IEEE Transactions on Wireless Communications, IEEE Internet of Things Journal, IEEE Wireless Communication Letters}, and \textit{China Communications}.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/DongfengYuan.png}}]{Dongfeng Yuan}(Senior Member, IEEE) received the M.S. degree from the Department of Electrical Engineering, Shandong University, China, in 1988, and received the Ph.D. degree from the Department of Electrical Engineering, Tsinghua University, China, in January 2000. Currently, he is a full professor in the School of Civil Engineering, Shandong University, China. From 1993 to 1994, he was with the Electrical and Computer Department at the University of Calgary, Alberta, Canada. He was with the Department of Electrical Engineering in the University of Erlangen, Germany, from 1998 to 1999; with the Department of Electrical Engineering and Computer Science in the University of Michigan, Ann Arbor, USA, from 2001 to 2002; with the Department of Electrical Engineering in Munich University of Technology, Germany, in 2005; and with the Department of Electrical Engineering Heriot-Watt University, UK, in 2006. His current research interests include Intelligent communication systems, mobile edge computing and cloud computing, AI and big data processing for communications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/xiaoyan_ma.jpg}}]{Xiaoyan Ma} received the B.S. degrees from the School of Information Science and Engineering, Shandong University, China, in 2017. She is currently pursuing her Ph.D. degree at the School of Information Science and Engineering, Shandong University, China. Her research interests include multiple-in multiple-out (MIMO) technology, reconfigurable intelligent surface (RIS) and machine learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/lidongyang.jpg}}]{Dongyang Li} received the B.E. and M.Eng. degrees in communication engineering from the School of Information Technology, Wuhan University of Technology, China, in 2015 and 2017, respectively. He is currently pursuing the Ph.D. degree with the School of Information Science and Engineering, Shandong University, China. His research interests include mobile edge computing, edge caching, federated learning, smart communication technologies.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/MinggaoZhang.png}}]{Minggao Zhang}
  received the B.Sc. degree in mathematics from Wuhan University, Wuhan, China, in 1962.  He was a Group Leader of the Radio Transmission Research Group, ITU-R, Geneva, Switzerland. He has been an Academician of Chinese Academy of Engineering, Beijing, China, since 1999. He is currently a Distinguished Professor with the School of Control Science and Engineering, Shandong University, Jinan, China, and a Senior Engineer of the 22nd Research Institute of China Electronics Technology Corporation, Xinxiang, China. He has been involved in the research of radio propagation for decades. Many of his proposals have been adopted by international standardization organizations, including CCIR P.617-1, ITU-R P.680-3, ITU-R P.531-5, ITUR P.529-2, and ITU-R P.676-3. Prof. Zhang is currently a fellow of the China Institute of Communications. He has received seven National and Ministerial Science and Technology awards in China. He has been an Academician with the Chinese Academy of Engineering since 1999. 
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> texes/intro_bak.tex <==


\section{Introduction}
\label{sec_intro}
 

%长时时间序列预测对很多实际应用具有十分重要的作用，例如能量和交通管理、经济和金融分析、传感器数据检测以及疾病传播预防等。因此，LTSF因其可以对较长时间范围的序列变化做出准确预测，近年来得到了广泛的关注。
%过去用于时间序列预测的深度学习方法包括RNN、LSTM等。这些方法对时序性进行了显示建模，也就是它当前时刻的输出除了基于其自身状态外，还依赖前一时刻的输出。这也使它们在处理LTSF任务时，更容易产生梯度消失或爆炸现象，因为需要计算更长、更复杂的梯度传播。

% 随着Transformer的到来，注意力机制被提出用来建模序列内部属性之间的依赖关系，从而解耦了模型对序列长度的依赖性，使其可以处理更长的序列。LogTrans通过因果卷积生成查询和键并按指数间隔来选择时间步长来减少原来Transformer的复杂度，它的复杂度为AA。Informer提出了ProbSparse注意力，通过将级联层输入减半来突出主导注意力同样也实现了AA的复杂度。FEDformer通过频率增强块来扩展Transformer，包括傅立叶增强块和小波增强块。通过随机选择固定数量的傅里叶分量，该模型实现了线性计算复杂度。



%Extending the forecasting time of time series is important for many practical applications, such as energy and traffic management, economic and financial analysis, sensor data detection, and disease propagation prevention. Therefore, 
Long-term Time Series Forecasting (LTSF) has received extensive attention in various domains, such as future energy and traffic management, extreme weather early warning, long-term economics and financial planning, etc. 
Extending the forecasting time is more challenging than traditional short-term prediction (e.g., one-step-ahead prediction) because the longer the forecast distance, the weaker the correlation of the time series, and the greater the uncertainty of the forecast results. 
Classical time series algorithms such as AR \cite{bollerslev1986generalized}, ARIMA \cite{li2012prediction} and VAR \cite{johansen1991estimation} etc. are no longer suitable for LTSF tasks, because their stationarity assumptions are only suitable for short-term and linearly dependent time series. 
To achieve longer time series forecasting, deep learning was introduced to process high-dimensional, non-stationary time series. 
Early deep learning methods for time series forecasting include recurrent neural networks (RNN) \cite{connor1994recurrent}, long short-term memory (LSTM) \cite{hochreiter1997long}, etc. 
These methods explicitly model the temporal dependencies of sequences, that is, their output at the current moment depends on the output at the previous moment in addition to their own state. This property also makes them more prone to vanishing or exploding gradients \cite{Glorot2010Understanding} when dealing with LTSF tasks, as longer and more complex gradient propagations need to be computed. 

\begin{figure}%[htbp]
  \centerline{\includegraphics[width=.5\textwidth]{figs/PF_Bubble_V4.pdf}}
  \caption{Performance (MSE), running time (Seconds/Epoch) and Flops (Bubble Size) comparison of Transformer-based models on the LTSF task. All models are Transformer-like architectures with 2-layer encoder and 1-layer decoder. Meanwhile, their input lengths are both 96, and their prediction lengths are 96, 192, 336, and 720, respectively. Periodformer is a Period-Attention based model proposed in this paper. Transformer, Informer and Autoformer are from \cite{NIPS2017_Transformer}, \cite{Zhou2021Informer} and \cite{wu2021autoformer}. Both Full-Attetnion and Prob-Attention models adopt the same architecture as Autoformer, but replace its attention part with Full-Attetnion \cite{NIPS2017_Transformer} and Prob-Attention \cite{wu2021autoformer}. All experiments were performed on the ETTm2 dataset using a Tesla V100 GPU, but similar results would be expected on other datasets or devices. The smaller the bubble and the closer it is to the bottom left corner, the better the overall performance of the model. Some models, such as FEDformer \cite{zhou2022fedformer}, were removed from this figure due to their long runtime (5$\times$ slower for FEDformer-f and 15$\times$ slower for FEDformer-w).}
  \label{fig1} % A lower MSE indicates a better performance. 
\end{figure}

% 所有模型的输入长度均为96，预测长度分别为96、192、336和720。它们的架构也都和Transformer相似，具有2层编码器和1层解码器。

With the advent of Transformer \cite{NIPS2017_Transformer}, attention mechanism is proposed to model the correlation between attributes within sequence, thereby decoupling the dependence of parameter on input length $L$, allowing it to handle longer sequence. 
However, the original attention has quadratic complexity $\mathcal{O}(L^2)$ when calculating the similarity between attributes, which is unaffordable for LTSF. 
Motivated by this, many works \cite{li2019enhancing, Kitaev2020Reformer, Zhou2021Informer, wu2021autoformer, zhou2022fedformer} have improved the attention mechanism to reduce its computational complexity. 
% For example, LogTrans \cite{li2019enhancing} reduces the complexity of the vanilla Transformer by generating queries and keys by causal convolution and selecting time steps at exponential intervals, which has a complexity of $\mathcal{O}(L{(logL)}^2)$. Reformer \cite{Kitaev2020Reformer} replaces the original dot-product attention by one that uses locality-sensitive hashing (LSH), which reduces the complexity to $\mathcal{O}(LlogL)$. Informer \cite{Zhou2021Informer} presents a KL-divergence based ProbSparse attention, which achieves $\mathcal{O}(LlogL)$ complexity by halving the cascaded layer input to highlight the dominant attention. Autoformer \cite{wu2021autoformer} designs an internal decomposition block and proposes an Auto-Correlation mechanism with information aggregation on Top-K similarity, which also achieves $\mathcal{O}(LlogL)$ complexity. FEDformer \cite{zhou2022fedformer} extends Transformer with frequency enhanced decomposed blocks, including Fourier enhanced blocks and Wavelet enhanced blocks. By randomly choosing a fixed number of Fourier components, FEDformer achieves linear computational complexity. 
These methods select time steps through operations such as exponential intervals (LogTrans \cite{li2019enhancing} with $\mathcal{O}(L{(logL)}^2)$), chunking (Reformer \cite{Kitaev2020Reformer} with $\mathcal{O}(LlogL)$), maximum activations (Informer \cite{Zhou2021Informer} with $\mathcal{O}(LlogL)$, Autoformer \cite{wu2021autoformer} with $\mathcal{O}(LlogL)$) or random sampling (FEDformer \cite{zhou2022fedformer} with $\mathcal{O}(L)$). They are all based on the vanilla Transformer, and discard some features to make the attention module sparse, thereby reducing the amount of computation. However, what we might wonder is

\textbf{Question 1: do these models actually reduce runtime while improving the performance on the LTSF task?} 

Our experiments show that the sparse attention mechanism designed by complex algorithms may not really reduce the running time of the model. On the contrary, the running time of the model may be increased due to the complex attention modules. As shown in Fig. \ref{fig1}, the vanilla Transformer may have less running time on real devices than other sparse attention-based models, but its performance on the LTSF task is very poor. Although some improved models, e.g., Informer, Autoformer, FEDformer, etc., theoretically reduce the computational complexity of Attention, they actually run slower and do not outperform the full-attention model using the same architecture. Further, another question we want to know about attention mechanism is

% in terms of performance
% 但是一个自然的问题是：这些模型真的降低了计算复杂度同时提高了模型在LTSF任务上的性能吗? 我们的实验表明，通过复杂的算法设计的稀疏注意力机制可能并没有真正的减少模型的复杂度。我们的实验表明通过复杂的算法设计的稀疏注意力机制可能并没有真正的减少模型的运行时间。反而，由于复杂的注意力机制可能会使模型的运行时间所有提高。
% 如图1所示，原来的具有二次计算复杂度的Transformer在真实设备上的运行时间可能比其他模型要少，但其在LTSF任务上的性能非常差。一些改进的模型虽然理论上减少了Attention的计算复杂度，但实际上却有着较慢的运行速度。

\begin{figure}%[htbp]
  \centerline{\includegraphics[width=.5\textwidth]{figs/PF_Trans_V4.pdf}}
  \caption{The vanilla Transformer performs poorly (lower than Autoformer) on the LTSF task. But if some improvements are made to Transformer, its performance (MSE, the lower the better) will be greatly changed. For example, adding moving average (Trans+MA) to reduce data noise, appropriately increasing Dropout (form 0.05 to 0.1) to change model sparsity will improve the average performance of Transformer. In particular, if Attention is removed (Trans$-$Att), the performance of the model will improve on some datasets, e.g., ETTm2, Exchange, etc., but will decrease on other datasets, e.g., Electricity, Traffic, etc.}
  \label{fig2} %  A lower MSE indicates a better performance. 
\end{figure}

\textbf{Question 2: Is the attention mechanism the key to improving the performance on the LTSF task?} 
% how important is the attention mechanism in improving the generalization of the model on the LTSF task?

The answer given by our experiments is that the effect of the attention module on the generalization of the model is diverse for different datasets. In this experiment, we first added the moving average (MA) module to Transformer to make it have the same architecture as Autoformer, which is denoted as Trans+MA. Then we remove all Attention modules from Trans+MA, denoted as Trans$-$Att, to compare their performance. As shown in Fig. \ref{fig2}, the performance of Trans$-$Att outperforms that of Autoformer with the same architecture on the ETTm2 dataset. But on the Electricity dataset, the performance of Trans$-$Att is worse than that of Autoformer. 
Another finding of this experiment is that the MA module for smoothing the input is critical to the performance improvement of the Transformer-based models on the LTSF task, suggesting that long inputs with high noise are detrimental to the generalization of the model on some datasets. However, existing models all take long inputs of the same length-$L$ to predict future long outputs of different lengths-$O$, denoting as $Input \text{-}L\text{-}predict\text{-}O$. So what we want to know about the input length is 

% 我们的实验给出的答案是，对于不同的数据集attention模块对模型的泛化的影响是不同的。在该实验中，我们首先对Transformer添加MA模块使它和Autoformer具有同样的架构，被记为Trans+MA。然后我们从Trans中去掉所有的Attention模块，记为Trans-Att，来对比它们的性能。
% 该实验的另一个发现是用于平滑输入的MA模块对基于Transformer的模型在LTSF任务上的性能提升非常关键，说明在某些数据集上似乎不需要太长的带有高噪声的输入。

\begin{figure}%[htbp]
  \centerline{\includegraphics[width=.5\textwidth]{figs/AT_Len+MA_V2.pdf}}
  \caption{Ablation experiments on the input length of the Trans+MA and the kernel size of the moving average (MA) module on the Exchange dataset. Trans+MA is an architecture similar to Autoformer obtained by adding the MA module to the vanilla Transformer. (a) Increasing the input length of Trans+MA will make its performance worse. (b) Increasing the kernel size of MA improves the average performance of Trans+MA when the input length is fixed. The input length is set to be 96 in this experiment. The numbers in the legend represent the forecast lengths, where the forecast errors are measured by MSE (dotted line) and MAE (solid line), respectively.}
  \label{fig3} %  A lower MSE indicates a better performance. 
\end{figure}


% Trans+MA是一种和Autoformer类似的架构，它是对原来的Transformer加上MA模块得到的。增加Trans+MA的输入长度会使其性能变差。当输入长度固定时，增加MA的核大小会使得Trans+MA的平均性能有所提升(但当预测长度为720时，性能下降)。
\textbf{Question 3: for LTSF, does the model need extra long input data to guarantee its performance?} 

Our experiments found that the input length of the model also has a direct impact on its performance. On some datasets, a short and efficient input length may be more effective than designing more complex models. As shown in Fig. \ref{fig3}, on the Exchange dataset, increasing the input length makes the average performance of Trans+MA worse. When the input is fixed, increasing the kernel size of the MA module improves the average performance of the model. 
%One exception is when the forecast length is equal to 720, the forecast error first increases and then decreases. 
This shows that the input length, the kernel size of MA and the prediction length are interrelated, and they jointly determine the final forecast performance. 
 

% 另一方面，时间序列的输入长短或许也影响着模型在不同数据集上的性能。然而，我们的实验发现在某些数据集上短且有效的输入或许比设计更复杂的模型更有效。
% 正如图3所示，在Exchange数据集上，增加输入长度会使得模型的平均性能变糟。当输入固定时，增加MV模块的核大小会使得模型的平均性能提升。
% 这说明输入长度，MA的核大小与预测长度是相互关联的，它们共同决定着最后的预测性能。



Based on the facts analyzed in Question 1 and Question 2, there are two issues that need further investigated: {\bf 1)} How to reduce the runtime of the attention mechanism on real devices and {\bf 2)} how to adjust its influence on the prediction results. 
The key to solving the above issues lies in the information aggregation strategies adopted by the attention mechanism, which are summarized in Fig. \ref{fig6}. 
%First, we start by analyzing the information aggregation strategies adopted by various attention mechanisms, as summarized in Fig. \ref{fig6}. 
% The information aggregation strategies adopted by various attention mechanisms are summarized in Fig. \ref{fig6}. 
The vanilla Transformer calculates attention scores for all moments in the series, which not only makes it have a quadratic computational complexity, but also makes it easier to fit irrelevant components in long-term series. 
The sparse attention version reduces computational complexity through random aggregation, but breaks the dependencies between sequences, making it difficult to guarantee better prediction results.
The frequency enhanced attention mechanisms (e.g. Autoformer and FEDFormer) exploit Fourier or Wavelet transform to compute the auto-correlation (implicit periodicity) of series to aggregate subseries. 
% These works compute the frequency components of the series through Fourier transform or Wavelet transform, and then obtain the implicit period of the series by selecting Top-K frequency components. 
However, harnessing Fourier or Wavelet transform into the attention mechanism will greatly increase its computational load, as the experimental results shown in Fig. \ref{fig1}. 

Motivated by this, we design a Period-Attention mechanism to achieve higher prediction performance with less computing resources, which is called Periodformer. As shown in \ref{fig6}, Periodformer renovates the aggregation of long-term subseries via explicit periodicity and short-term subseries within the period via built-in proximity. It not only alleviates the repeated aggregation of some irrelevant series components, but also avoids some time-consuming frequency transformations. This property makes it have a linear computational complexity, which guarantees fast running speed on real devices. Meanwhile, a gate mechanism is built into the Period-Attention module, which adopts a scaling factor to adjust the influence of the attention score to its output. This mechanism makes Period-Attention have high flexibility, thus making full use of its sequence modelling capabilities and reducing its negative impact on prediction results. 

% For example, Autoformer and FEDFormer exploit the decomposition \cite{1976_timeseries, 1990stl} and implicit periodicity of time series to model the relationship between different moments.

% 根据问题1和问题2的答案，我们需要设计一种在真实设备上运行时间短并且对预测结果的影响是可调节的注意力机制。传统的注意力机制对序列中的所有时刻计算注意力得分，这不仅使其具有二次方的计算复杂度，同时使其更容易拟合长时间序列中的无关分量。因此，一些方法利用时间序列的分解通过其周期性来显式建模不同时刻的关系。这些工作通过傅里叶变换或小波变换来计算序列的频率分量，然后通过选择Top-K的频率分量来得到序列的隐式周期。然而，在注意力机制里面内置傅里叶变换或小波变换会极大地增加其计算负载。因此，我们设计了一种基于周期的注意力机制真正地实现了使用更少计算资源取得更高预测性能的目的。Periodformer基于序列的周期相似性来聚合信息，而在同一周期内只利用序列的局部相似性。周期注意力对模型的影响是可调的，且具有线性的计算复杂度，使其具有足够的灵活性以及快速的运行速度。

According to the facts analyzed in Question 3, we need to find suitable hyperparameters for the input length and the kernel size of MA to achieve better generalization. However, hyperparameter search is a very time-consuming task. The existing hyperparameter search methods are all based on CPU to provide parallel search for traditional learning models, or provide hyperparameter search for deep learning models based on single GPU or multi-GPU single process. These methods cannot distribute the deep learning model and its hyperparameters to multiple GPUs for asynchronous parallel search, thus failing to accelerate the search process. 
Therefore, we design a Multi-GPU Asynchronous parallel hyperparameter search algorithm based on Bayesian Optimization (BO) to perform fast hyperparameter search for deep learning models, which is called MABO. This algorithm allocates a process to each GPU through a queue mechanism, and then creates multiple trials (including data, models and its hyperparameters) at a time for asynchronous parallel search. It can quickly find suitable hyperparameters (i.e. input length, kernel size of MA and  scaling factor of Period-Attention, etc.), which greatly reduces the search time.

%The algorithm distributes the deep learning model and its hyperparameters to multiple GPUs for asynchronous parallel search, which greatly accelerates the process of hyperparameter search. 

%  MABO is used to search hyperparameters such as the input length of the model, the scaling factor of the period-attention and the kernel size of the MA. 

% 根根据问题3的答案，我们需要为输入长度和MA的核大小寻找合适的超参数来取得更好的泛化性。然而，超参数搜索是一个十分耗时的任务。现有的超参数搜索方法基于CPU来进行并行搜索或者基于单GPU多线程、多GPU单进程进行搜索。 这些方法无法将深度学习模型及其超参数分发到多GPU上进行异步并行搜索，因而无法加速其搜索过程。
% 因此，我们设计了一种多GPU异步并行的超参数优化算法来进行快速的超参数搜索。MABO被用来对Periodformer的输入长度，period的缩放因子以及MA的核大小等超参数进行搜索。它将模型分发到多个GPU上进行超参数搜索，极大地加速了超参数搜索的过程。


\textbf{The main contributions are summarized as the following.}
\begin{itemize} %[leftmargin=*]
  \item It is found that the traditional attention-based LTSF methods only theoretically reduce their computational complexity, but do not reduce the running time on practical devices. Meanwhile, it is found that both the input length of the series and the kernel size of the MA have a direct impact on the final forecast.
  \item A period-based attention mechanism (Periodformer) is proposed, which renovates the aggregation of long-term subseries via explicit periodicity and short-term subseries via built-in proximity. These properties make it have a linear computational complexity, which guarantees high predictive performance and fast running speed on real devices.
  \item A multi-GPU asynchronous parallel hyperparameter search algorithm based on Bayesian optimization (MABO) is presented to find suitable hyperparameters. MABO allocates a process to each GPU via a queue mechanism, and then creates multiple trials at a time for asynchronous parallel search, which greatly accelerates the search process.
  \item Periodformer has a good generalization on many LTSF tasks, and experimental results reveal that the proposed method achieves SOTA performance and provide strong benchmarks.

\end{itemize}



% 我们发现传统的基于注意力的LTSF方法，只是在理论上降低了其计算复杂度，但在实际设备上却并没有减少运行时间。
% 一种基于周期的注意力机制被提出，该模块基于周期来聚合长时性信息，并基于局部性来聚合短时性信息。
% 一种基于周期的注意机制被提出，它基于周期性聚合长期信息，基于局部性聚合短期信息。AAA具有线性的计算复杂度，保证了其具有较高的预测性能同时在真实设备上有较快的运行速度。
% 我们呈现了一种基于贝叶斯优化的多GPU异步并行超参数搜索算法来寻找合适的超参数。该算法将模型及其超参数分发到多个GPU上进行异步搜索，极大地加速了超参数的搜索过程。


The remaining of the paper is organized as follows. In Section \ref{sec_pf}, the architecture of Periodformer and Period-Attention mechanism will be introduced in detail. In Section \ref{sec_mabo}, MABO and its algorithm will be introduced. Section \ref{sec_exp} introduces experimental results of the proposed method and Section \ref{sec_rework} summarizes related work. Finally, we conclude the paper in Section \ref{sec_con}.


\begin{figure}%[htbp]
  \centerline{\includegraphics[width=.5\textwidth]{figs/Fig3_2.pdf}}
  \caption{Information aggregation strategies adopted by various attention mechanisms. Full Attention \cite{NIPS2017_Transformer} (a) aggregates information from all moments. Sparse Attention \cite{li2019enhancing, Kitaev2020Reformer} (b) aggregates information through fixed intervals or random sampling. Auto-Correlation \cite{wu2021autoformer} (c) aggregates information through the implicit periodicity obtained by Fourier transform. Period-Attention (ours) (d) aggregates information based on the explicit periodicity of series.} 
  \label{fig6} 
\end{figure}

% 各种注意力机制所采用的信息聚合策略。全注意力聚合了所有时刻的信息。稀疏注意力通过随机采样或固定间隔来进行信息聚合。
